Is the EJRA proportionate and therefore justified? A critical review of the EJRA policy at Cambridge

This paper critically evaluates the HESA (Higher Education Statistics Agency) Data Report for the Employer Justified Retirement Age (EJRA) Review Group at the University of Cambridge (\cite{CambridgeHESA2024}), identifying significant methodological flaws and misinterpretations. Our analysis reveals issues such as unclear application of data filters, inconsistent variable treatment, and erroneous statistical conclusions. The Report suggests that the EJRA increased job creation rates at Cambridge, but we show Cambridge consistently had lower job creation rates for Established Academic Careers compared to other Russell Group universities, both before and after EJRA implementation in 2011, with no evidence for a significant change in this deficit post implementation. This suggests that EJRA is not a significant factor driving job creation rates. Since other universities without an EJRA exhibit higher job creation rates, this suggests job creation can be sustained without such a policy. We conclude that the EJRA did not achieve its intended goal of increasing opportunities for young academics and may have exacerbated existing disparities compared to other leading universities. We recommend EJRA be abolished at Cambridge since it does not meet its aims and could be viewed as unlawful age discrimination.\newline \it{This version is a revision reflecting some of the comments made by members of the university EJRA review group in public discussion, see \cite{Holmes24}.}

==> background.tex <==
\section{Background}

%Universities worldwide face significant challenges in hiring and retaining high-quality faculty members due to the problems of information asymmetry, specifically adverse selection and moral hazard. Adverse selection arises \textit{before} hiring, as universities struggle to accurately assess candidates' true qualifications, potential for research excellence, and teaching effectiveness. Despite rigorous selection processes, applicants may misrepresent their abilities by highlighting successful projects while downplaying or omitting less favorable outcomes. This information gap can lead to hiring individuals who do not optimally meet the institution's needs.

%Moral hazard, in contrast, manifests \textit{after} hiring, as the interests of faculty members may diverge from those of the university due to the security provided by tenure. Once hired, some faculty may not maintain the expected standards of performance, especially after securing tenure or long-term contracts, knowing their positions are secure regardless of their efforts. This can lead to a reduction in research output, teaching quality, or a lack of engagement in institutional service activities.


% Cambridge hires and places people on the global market so in terms of assisting young people by creating jobs the contribution to global vacancies is minimal. Also, named professorships of which there are many are filled by senior people from worldwide so many of the vacancies will not be for young people living within 5 miles of St. Marys church.

%When the coalition government abolished the default retirement age in 2011, they produced an economic impact statement where their central estimate was that getting rid of retirement would unleash \pounds 2.5billion dollars benefit to the economy as a whole in the medium run. This was based on allowing people to continue working when they were still productive and wanted to continue and the expansion of the labour supply that it entailed. They also quantified some benefit to the exchequer from the taxes that would be paid and the reduction in benefits that would have to be paid. Most universities now have on their websites claims about how much they contribute to the UK economy and the balance of payments and so on. How much more could Cambridge contribute if it abolished the EJRA.

Universities face significant information asymmetry problems when hiring faculty. Universities may not have full information about a candidate's true abilities, research potential, teaching effectiveness, etc. Specifically, there are two problems that universities attempt to address through their hiring practices: Adverse selection and moral hazard. 

Adverse selection in faculty hiring occurs before the candidate is hired, specifically because universities face challenges in accurately assessing the true qualifications and potential of candidates. Candidates may misrepresent their abilities, highlighting their most successful projects while downplaying or omitting less successful ones, leading to the hiring of individuals who do not meet the institution's needs as effectively as their applications suggest. Additionally, universities often rely on proxies such as the reputation of the candidate’s alma mater or previous institutions, which can result in hiring candidates from prestigious institutions who may not necessarily be the best fit for the specific needs of the hiring department. The diverse and sometimes conflicting criteria for evaluating candidates, such as research excellence versus teaching effectiveness, further complicate the selection process. Moreover, candidates with interdisciplinary expertise may be undervalued if search committees are not equipped to assess contributions outside their primary discipline, leading to a preference for candidates with more traditional, easily recognizable qualifications. 

In contrast, moral hazard in faculty hiring arises after the candidate is hired, specifically because the actions of faculty members post-hiring are not fully aligned with the interests of the university, primarily due to the security provided by tenure. Once hired, faculty members might not perform to the expected standards, especially if they have secured tenure or a long-term contract, knowing that their job is secure regardless of their performance. This can lead to a reduction in research output or teaching quality. The tenure system itself can create moral hazard by providing job security without sufficient accountability, allowing faculty members to slack off once they achieve tenure. Additionally, faculty members might exploit the resources provided by the university, such as research funds and lab space, without delivering commensurate results, especially if there is insufficient oversight or accountability mechanisms in place. 

To solve these two problems, universities especially in the United States, grant tenure following a probation period. At the end of the probation period, the candidate is evaluated. The probation period allows the university to solve the adverse selection problem by not committing to retain the employee if the employee does not perform in a five to six year window. At the end of the window, the candidate is either promoted with tenure or fired, in a rule called an up-or-out rule. The up-or-out rule solves a double-sided moral hazard problem. The employer sets a wage higher than opportunity cost to induce the worker to invest in firm-specific capital. The university solves one side of the moral hazard problem by setting high standards. If the individual does not make the grade, it is in the firm’s interest ex post to fire him. However, had the initial arrangement not included provisions for firing individuals, the firm would underreport the value of the employee, which would destroy the incentive scheme (\cite{KahnHuberman1988}).

On passing the review process, in the US academic system, the faculty member is tenured. Tenure is a contractual right not to have the position terminated without just cause. To put it simply, a tenured professor cannot be fired unless he/she does something illegal. Prima facie, this concept appears untenable in the 21st century. With widespread job insecurity even among the highly educated, it appears archaic that a particular group of employees, university faculty, are given life-time employment. In the US, tenure is sharply binary – a handful of scholars get tenure while a large number of academics get poorly paid non-tenured posts with little status or security (\cite{Rau2014FT}).

Proponents of tenure argue that tenure preserves the quality of university education, since it gives professors academic freedom to pursue path-breaking research ideas and to freely voice their own opinions without being censured by administrators. Opponents of tenure argue that tenure is part of an outmoded system that encourages professors to pursue research, usually of questionable quality, over teaching. Some opponents argue that tenure actually reduces academic freedom because to get tenure, academics must conform to the political or academic mainstream.

From an economic point of view however, tenure can be seen as a simple mechanism for universities to assure themselves of quality research. Tenure is a way for universities to solve both information asymmmetry problems: first, they need to hire faculty who will be research active in the long term – the adverse selection problem. Second, they need to make sure that they offer incentives for the faculty to stay research active once hired – the moral hazard problem. 

Once a professor gains tenure, he/she cannot be fired. So the tenure process would seem to exacerbate the moral hazard problem. If the university can do nothing to punish the professor, a tenured professor can slack off the rest of his/her life without fear. A regular system of performance reviews might appear to be better than tenure here – if a professor starts slacking off, he will be fired on his next review.

However, this system makes the adverse selection process worse – and adverse selection is the primary concern for the university. Consider what it is that makes a university’s reputation. Great teachers are memorable to their students, but what really makes a university famous is the quality of its research. What did professors at the university discover? What did they create? This is what we remember the great universities for. The annual university reputation rankings published by the Times Higher Education group (\cite{THE2023}) for example, give twice the weight to research as to teaching. Teaching is measurable. The quality of teachers can be assessed through student evaluations, student signups for elective classes, and so on. 

However, basic research by its very nature, is unpredictable. Science has become increasingly specialized, so much so, that a scientist in one field will not be able to understand why a discovery in another field is important if at all. If an economics professor shows her  latest paper to a sociologist, the sociologist is likely to look completely blank. This means that the best judges of quality are other professors in the same field. 

Now suppose a university were to abolish tenure. Instead it announces that every five years, there will be a performance review and the ones who have contributed least to research will be fired (the university will not put that much emphasis on teaching because as noted above, its reputation depends on the ideas that professors generate). Now what is the best strategy for a senior untenured professor in the area? Simple. Interview all the aspiring professors and hire the idiots. In five years, the new untenured professors will all be fired because ex ante they had silly research ideas and the wise senior professor achieves de facto, though not de jure, tenure. That is the adverse selection problem the university faces. To solve it, the university says to the senior professor, hire the smart juniors. They will bring fame to the department, bring in more funds from government and industry, and increase the resources available to you. But your job is safe whatever happens.

Unfortunately, this worsens the moral hazard problem. So how do universities solve that problem? They make the tenure process so difficult that only a handful of professors achieve it. In the US system, over 90\% of professors do not make tenure in the schools they start in. Why do universities make this hurdle so high? That is because universities hope that the handful of professors who do achieve tenure are so driven that they will work hard even though they do not have to. Though of course, the university acknowledges that this is a hope, not a requirement.

If the hope is not fulfilled, the university has academic deadwood on its hands. How does it get rid of the deadwood? U.S. universities do this by either buying out the deadwood (offering them a generous deal to leave early) or treating them so harshly (assign them teaching at unreasonable hours, force them to offer new preps every year and so on) that they leave on their own.

The University of Cambridge in the United Kingdom (U.K.) follows a different path. Rather than implement an effective performance management system (without getting rid of the tenure process, which, recall would be detrimental to the university), it has chosen to use an Employer-Justified Retirement Age (EJRA) that is currently set at 67 years. Simply put, all academic staff of the university are forcibly retired at 67 years.
